Equiformer: Equivariant Graph Attention Transformer for 3D Atomistic Graphs

Despite their widespread success in various domains, Transformer networks have yet to perform well across datasets in the domain of 3D atomistic graphs such as molecules even when 3D-related inductive biases like translational invariance and rotational equivariance are considered. In this paper, we demonstrate that Transformers can generalize well to 3D atomistic graphs and present Equiformer, a graph neural network leveraging the strength of Transformer architectures and incorporating SE(3)/E(3)-equivariant features based on irreducible representations (irreps). First, we propose a simple and effective architecture by only replacing original operations in Transformers with their equivariant counterparts and including tensor products. Using equivariant operations enables encoding equivariant information in channels of irreps features without complicating graph structures. With minimal modifications to Transformers, this architecture has already achieved strong empirical results. Second, we propose a novel attention mechanism called equivariant graph attention, which improves upon typical attention in Transformers through replacing dot product attention with multi-layer perceptron attention and including non-linear message passing. With these two innovations, Equiformer achieves competitive results to previous models on QM9, MD17 and OC20 datasets.

==> content/2_1_graph_neural_networks_and_3d_graph.tex <==
\vspace{-1mm}
\subsection{Graph Neural Networks}
\vspace{-1mm}

Formally, a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ consists of nodes $i \in \mathcal{V}$ and edges $(i, j) \in \mathcal{E}$ representing relationships between nodes $i$ and $j$. 
%We can use graphs to represent atomistic systems like molecules, where nodes are atoms and edges can represent bonds or geometric relationships between two atoms \tess{; we refer to these as atomistic graphs}.
Graphs can represent atomistic systems like molecules, where nodes are atoms and edges can represent bonds or atom pairs within a certain distance; we refer to these as atomistic graphs. % \tess{; we refer to these as atomistic graphs}.
%Each node has associated features $f_i$, and each edge has features $e_{ij}$.
Graph neural networks (GNNs) \revision{generally} extract meaningful representations from graphs through message-passing layers.
Given feature $f_i^{l}$ on node $i$ and edge feature $e_{ij} ^ l$ at the $l$-th layer, it first aggregates messages $m_{ij}^l$ from neighbors and then update features on each node as follows:
\begin{equation}
%\begin{split}
m_{ij}^l = \phi_{m}(f_i^{l}, f_j^{l}, e_{ij}^{l}) 
\quad\text{and}\quad
f_{i}^{l+1} = \phi_{u}(f_{i}^{l}, \sum_{j \in \mathcal{N}(i)} m_{ij}^{l} )
%\end{split}
\end{equation}
where $\mathcal{N}(i)$ denotes the set of neighbors of node $i$ and $\phi_m$ and $\phi_u$ are learnable functions.
For atomistic systems in 3D spaces, each node $i$ is additionally associated with its position $\vec{r_i}$ and typically edge features become functions of relative position $\vec{r}_{ij} = \vec{r}_j - \vec{r}_i$.
%; we refer to these as \revision{3D} atomistic graphs.


==> content/2_5_e3_equivariant_neural_networks.tex <==
\vspace{-1mm}
\subsection{$E(3)$-Equivariant Neural Networks}
\vspace{-1mm}

$E(3)$-equivariant neural networks (ENNs) are built such that every operation $f$ is equivariant to Euclidean symmetry, satisfying that for $g \in E(3)$, inputs $x$ and scalar weights $w$ and $f:X \times W \rightarrow Y$, $f(D_X(g)x, w) = D_Y(g)f(x, w)$ \cite{tfn,kondor2018clebsch,3dsteerable}.
In addition to the tensor product, equivariant operations also include equivariant activation functions and normalizations as in typical neural networks, and we discuss those used in Equiformer in Sec.~\ref{subsec:equivariant_operations}.


%%%%%%%%%%%%%%%%%%

%Because an ENN is a composition of equivariant operations, it is also equivariant; transformations acting on input spaces propagate to the output spaces, e.g., when we rotate an input atomistic graph, predicted vectors will be rotated.




% \revision{Since each operation is equivariant, the whole networks can propagate transformation acting on input spaces to output spaces and achieve equivariance, e.g., when we rotate an input atomistic graph, predicted vectors will be rotated by design.}
%\revision{There have been several works leveraging equivariant networks~\cite{tfn, 3dsteerable, kondor2018clebsch, l1net, nequip, se3_transformer, segnn, allergo} for different applications such as energy prediction~\cite{tfn, se3_transformer, segnn} and molecular dynamics~\cite{nequip, allergo}.}
%\todo{Typical equivariant operations beyond tensor product (e.g., activation and linear).}
%\todo{How we stack equivariant operations to build equivariant networks.}
%\todo{Some typical examples.}

==> content/3_1_incorporatting_e3_representations.tex <==
\subsection{Incorporating E(3) Features}
\label{subsec:incorporate_e3_features}

\begin{figure*}[t]
\includegraphics[width=0.9\linewidth]{figure/equiformer.png}
\centering
\caption{\textbf{Architecture of Equiformer.}
\todo{Add detailed explanation of each submodule of Attention to figures in Appendix.}
\todo{Add dot product attention in Appendix.}
\todo{Update variables: $x_{ij}, a_{ij}, v_{ij}$}
Here ``$\otimes$'' denotes multiplication, ``$\oplus$'' denotes addition, and ``DTP'' stands for depth-wise tensor product. $\sum$ within a circle denotes summation over all neighbors.
}
\label{fig:equiformer}
\end{figure*}

\begin{enumerate}
    \item \note{Typical GNN and Transformer operate on scalars}
    \item \note{Equivariance}
    \item \note{Including E(3)}
    \item \note{Picture for Linear, Gate, DTP, Layer Norm}
\end{enumerate}

\todo{May be moved to Background}

\todo{Definition of Graph and 3D Graph}


\paragraph{Directional Information.}
Typical graph neural networks (GNNs) use scalars as internal representations.
As scalars are invariant features, after geometric transformations like rotations, they will remain the same.
This means that the representations are insensitive to rotations and therefore cannot encode any directional information.
However, directional information contained in quantities like forces is indispensable to understand interactions between atoms from the perspective of physics.
Moreover, discarding directional information can make GNNs less expressive as they cannot differentiate certain types of graphs.
These motivate using other representations instead of only scalars.


\paragraph{Equivariance.}

\paragraph{E(3) Features.}


==> content/3_4_edge_degree_embedding.tex <==
\begin{wrapfigure}[8]{r}{0.25\textwidth}
\vspace{-1.0em}\centering\strut
%\includegraphics[width=0.4\textwidth,clip,trim=1cm 2.5cm 1cm 1cm]{figs/teasers/teaser-computation-v2.pdf}
\includegraphics[width=0.2\textwidth]{figure/attention_not_distinguish.png}
\vspace{-0.5em}
\caption{\textbf{Examples of graphs hard for pure attention to distinguish.}}
\label{fig:attention_not_distinguish}
\end{wrapfigure}

\subsection{Edge-Degree Embedding}
\label{subsec:edge_degree_embedding}


Softmax in equivariant graph attention calculates weighted averages over all neighboring nodes.
Therefore, there exist some cases where attention cannot distinguish between two different graphs.
For example, the two graphs in Fig.~\ref{fig:attention_not_distinguish} cannot be distinguished by attention if we only consider scalars and features on nodes of the same colors are identical.
This results in the same output of attention for two different graphs.

Degree information is indispensable to differentiate between the two graphs, and therefore, we propose edge-degree embedding to address the issue.
As depicted in the right branch in  Fig.~\ref{fig:equiformer}(c), we first transform a constant one vector into messages encoding local geometry with two linear layer and one intermediate DTP layer.
The DTP layer has the same form as that in Eq.~\ref{eq:pre_attn}.
We then use sum aggregation~\cite{gin} to encode degree information.
We scale the aggregated features by dividing with the squared root of average degrees in training sets so that standard deviation of aggregated features would be close to $1$.
Including degree information can easily differentiate the two graphs, and therefore, we place edge-degree embedding at the beginning of Equiformer.

==> content/7_checklist.tex <==

\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include code related to experiments on QM9 in supplementary. Code reproducing all experiments will be available.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{As each experiment takes much time, we are not able to run several times. However, the proposed method improves upon previous works by a clear margin, and therefore the improvement is not within noise ranges.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


